ReLANCE: A Resource-Efficient Low-Latency Cortical Neural Acceleration Engine

We present a Cortical Neural Pool (CNP) architecture featuring a high-speed, resource-efficient CORDIC based Hodgkin-Huxley (RCHH) neuron model. Unlike shared CORDIC-based DNN approaches, the proposed neuron leverages modular and performance-optimised CORDIC stages with a latency-area trade-off. We introduce a novel Constraint-Aware Modular Parallelism (CAMP) with Precision & Stability handling to leverage maximum speedup and utilisation of hardware through hardware software co-design. The FPGA implementation of the RCHH neuron shows 24.5% LUT reduction and 35.2% improved speed, compared to SoTA designs, with 70% better normalised root mean square error (NRMSE). Furthermore, the CNP exhibits 2.85x higher throughput (12.69 GOPS) than a functionally equivalent CORDIC-based DNN engine, with only a 0.35% accuracy drop relative to the DNN counterpart on the MNIST dataset. The overall results indicate that the design shows biologically accurate, low-resource spiking neural network implementations for resource-constrained edge AI applications. The reproducibility codes are publicly available at https://github.com/mukullokhande99/CNP RCHH, facilitating rapid integration and further development by researchers.

==> impl.tex <==
{\fontsize{10.5pt}{12pt}\selectfont Here, we implement COordinate Rotation Digital Computer, CORDIC, in short, to replace complex operations like multipliers in the HH model. CORDIC, in short, is a rotation-based iterative algorithm, mostly used to replace complex multiplications with simpler shifters and adders iteratively. We do not arrive at the precise value, but a close enough approximation of the desired value. This is done by adjusting the CORDIC iterations to achieve the desired accuracy. We have implemented three CORDIC cores for multiplication, division, and exponential operation. Here's a top-level algorithmic/ logical flow of each to understand CORDIC intuitively:
\vspace{-6pt}
\subsubsection*{\fontsize{8.5pt}{9pt}\selectfont \textcolor{blue}{CORDIC EXPONENTIAL}}
\vspace{-5pt}
{\fontsize{10.5pt}{12pt}\selectfont The CORDIC exponential algorithm computes $e^{p}$ using an iterative approach that breaks down the computation of $e^{{p_{frac}}+{p_{int}}}$ into two phases:
\newline
\textbf{Phase 1 ($e^{p_{frac}}$):} We start with the result $r(0) = 1$, (implicit initialization), then for each iteration $j$ from $-k$ to $-1$, we check if $p_{frac}$ is larger than $2^{-i}$ (Here $k$ refers to total number of CORDIC exponential iterations). If yes, we subtract $2^{-j}$ from $p_{frac}$ and multiply $r$ by $a(i) = e^{2^{-j}}$ (precomputed and stored in an LUT). This effectively builds up $p_{frac}$ by selecting appropriate powers of $e$.
\newline
\textbf{Phase 2 ($e^{p_{int}}$):} This is much more simpler. Here If  $p_{int}$ > 0, we multiply $r$ by $e$ and decrement $p_{int}$. If $p_{int}$ < 0, we divide $r$ by $e$ and increment $p_{int}$. We continue this until $p_{int}$ = 0.}
\vspace{-6pt}
\subsubsection*{\fontsize{8.5pt}{9pt}\selectfont \textcolor{blue}{CORDIC MULTIPLICATION}}
\vspace{-5pt}
{\fontsize{10.5pt}{12pt}\selectfont For the product of two numbers, $r = p \times q$, the multiplier $p$ is iteratively decomposed into a sum of powers of two ($2^{-j}$). In each iteration $j$, the algorithm checks a condition on the remainder of $p$. If the condition is met, $2^{-j}$ is subtracted from the remainder of $p$, and ($q \times 2^{-j}$) is added to the running total, $r$. This process continues until the remainder of $p$ is driven to zero.}
\vspace{-6pt}
\subsubsection*{\fontsize{8.5pt}{9pt}\selectfont \textcolor{blue}{CORDIC DIVISION}}
\vspace{-5pt}
{\fontsize{10.5pt}{12pt}\selectfont For the quotient $r = p/q$, in each iteration $i$, a scaled version of the divisor, $q \times 2^{-j}$, is conditionally subtracted from or added (based on the sign of the remainder, $p$) to the remainder ($p$, acts as a running reminder). If the subtraction is possible without the remainder changing sign, $2^{-j}$, is added to the quotient, $r$. This process continues until the remainder goes to zero.}

\begin{figure}[htbp]
\centering
% --- LEFT COLUMN (Algorithm 1: Exponential) ---
\begin{minipage}[b]{0.5\textwidth} % <-- CHANGED to [b] for bottom alignment
    \begin{algorithm}[H]
    \caption{CORDIC Exponential}
    \label{alg:cordic_exp}
    \begin{algorithmic}[1]
        \State Decompose $p \to p_{\text{int}} + p_{\text{frac}}$
        \State Initialize $r(0) \gets 1$
        \Statex
        \State \textbf{Phase 1: Compute $e^{p_{\text{frac}}}$}
        \For{$j \gets -k$ to $-1$}
            \If{$p_{\text{frac}}(j) > 2^{-j}$}
                \State $p_{\text{frac}}(j+1) \gets p_{\text{frac}}(j) - 2^{-j}$
                \State $r(j+1) \gets r(j) \times a(j)$
            \EndIf
        \EndFor
        \Statex
        \State \textbf{Phase 2: Handle $e^{p_{\text{int}}}$}
        \While{$p_{\text{int}}(j) \ne 0$}
            \If{$p_{\text{int}}(j) > 0$}
                \State $r(j+1) \gets r(j) \times e$
                \State $p_{\text{int}}(j) \gets p_{\text{int}}(j) - 1$
            \Else
                \State $r(j+1) \gets r(j) / e$
                \State $p_{\text{int}}(j) \gets p_{\text{int}}(j) + 1$
            \EndIf
        \EndWhile
        \State\Return $r$
    \end{algorithmic}
    \end{algorithm}
\end{minipage}
\hfill % Pushes the two columns apart
% --- RIGHT COLUMN (Algorithms 2 & 3) ---
\begin{minipage}[b]{0.45\textwidth} % <-- CHANGED to [b] for bottom alignment
    % Algorithm 2: Division
    \begin{algorithm}[H]
    \caption{CORDIC Division}
    \label{alg:cordic_div}
    \begin{algorithmic}[1]
        \For{$j \gets -k$ to $k$}
            \If{$p(j) \ge 0$}
                \State $p(j+1) \gets p(j) - 2^{-j} \times q$
                \State $r(j+1) \gets r(j) + 2^{-j}$
            \Else
                \State $p(j+1) \gets p(j) + 2^{-j} \times q$
                \State $r(j+1) \gets r(j) - 2^{-j}$
            \EndIf
        \EndFor
    \end{algorithmic}
    \end{algorithm}
    \vfill % <-- CHANGED to \vfill to push Algorithm 3 down
    % Algorithm 3: Multiplication
    \begin{algorithm}[H]
    \caption{CORDIC Multiplication}
    \label{alg:cordic_mult}
    \begin{algorithmic}[1]
        \For{$j \gets -l$ to $k$}
            \If{$p(j) \ge 0$}
                \State $p(j+1) \gets p(j) - 2^{-j}$
                \State $r(j+1) \gets r(j) + 2^{-j} \times q$
            \Else
                \State $p(j+1) \gets p(j) + 2^{-j}$
                \State $r(j+1) \gets r(j) - 2^{-j} \times q$
            \EndIf
        \EndFor
    \end{algorithmic}
    \end{algorithm}
\end{minipage}
\end{figure}
}
{\fontsize{10.5pt}{12pt}\selectfont
These CORDIC cores are primarily used in rate calculations (Table~\ref{tab:rate_constants}), making them hardware-efficient while retaining \textbf{accuracy} of up to \(\bm{\le 0.5\%\text{--}1\%}\) with increased iterations (\(\bm{14}\) for multiplication, \(\bm{8}\) for division, and \(\bm{12}\) for exponential). Here, a \(\bm{22\text{-bit}\ Q10.12}\) fixed-point representation is implemented. The voltage update and spike detection mechanism remains the same as in equation 1. The neuron solver is controlled by a top FSM (Fig.~\ref{fig:3}), where each state triggers a dedicated sub-FSM for a particular computation (e.g., rate calculation and power calculation stages, which use CORDIC readily). The FSM diagram (Fig.~\ref{fig:3}) clearly illustrates these transitions: rate calculation, power calculation, current calculation, and update. 

